Adolescent sports participation and health in early adulthood: An observational study

We study the impact of teenage sports participation on early-adulthood health using longitudinal data from the National Study of Youth and Religion. We focus on two primary outcomes measured at ages 23--28 -- self-rated health and total score on the PHQ9 Patient Depression Questionnaire -- and control for several potential confounders related to demographics and family socioeconomic status. To probe the possibility that certain types of sports participation may have larger effects on health than others, we conduct a matched observational study at each level within a hierarchy of exposures. Our hierarchy ranges from broadly defined exposures (e.g., participation in any organized after-school activity) to narrow (e.g., participation in collision sports). We deployed an ordered testing approach that exploits the hierarchical relationships between our exposure definitions to perform our analyses while maintaining a fixed family-wise error rate. Compared to teenagers who did not participate in any after-school activities, those who participated in sports had statistically significantly better self-rated and mental health outcomes in early adulthood.

==> health_table.tex <==
% latex table generated in R 4.3.2 by xtable 1.8-4 package
% Sun Feb 18 15:09:23 2024
\begin{table}[ht]
\centering
\begin{tabular}{llrrll}
  \hline
Exposure & Decision & p-value & Estimate & CI (marginal) & CI (corrected) \\ 
  \hline
any activity & Rejected & 0.01 & 0.07 & (0.01, 0.13) & (0.01, 0.13) \\ 
  any sports & Rejected & 0.01 & 0.07 & (0.01, 0.13) & (0.01, 0.13) \\ 
  no sports & Not Rejected & 0.08 & 0.05 & (-0.01, 0.12) & (-0.03, 0.13) \\ 
  any contact & Rejected & 0.01 & 0.08 & (0.01, 0.14) & (0.01, 0.15) \\ 
  no contact & Not Rejected & 0.35 & 0.05 & (-0.07, 0.15) & (-0.09, 0.17) \\ 
  any collision & Not Rejected & 0.17 & 0.06 & (-0.04, 0.15) & (-0.05, 0.17) \\ 
  no collision & Not Rejected & 0.03 & 0.07 & (-0.00, 0.15) & (-0.01, 0.16) \\ 
   \hline
\end{tabular}
\caption{Hypothesis testing for self-rated health} 
\label{tab:health_bin}
\end{table}


==> hypothesis_table.tex <==
\begin{table}[ht]
    \centering
    \begin{tabular}{rll}
    \hline
    Null Hypothesis & Explanation & Type-I error\\ 
    \hline
    $H_0^{(1)}: \tau^{(1)} = 0$ & No effect of any activity vs no activity & $\alpha$\\
	$H_0^{(2)}: \tau^{(2)} = 0$ & No effect of any sports activities vs no activity & $\alpha$\\
	$H_0^{(3)}: \tau^{(3)} = 0$ & No effect of non-sports activities vs no activity & $\alpha/3$\\
	$H_0^{(4)}: \tau^{(4)} = 0$ & No effect of contact sports vs no activity & $2\alpha/3$\\
	$H_0^{(5)}: \tau^{(5)} = 0$ & No effect of non-contact sports vs no activity & $\alpha/3$\\
	$H_0^{(8)}: \tau^{(8)} = 0$ & No effect of collision sports vs no activity & $\alpha/3$\\
	$H_0^{(9)}: \tau^{(9)} = 0$ & No effect of non-collision sports vs no activity & $\alpha/3$\\
    \hline
    \end{tabular}
    \caption{Hypotheses to be tested along with the type-I error allowable for each test to maintain a family wise error rate of $\alpha$}
    \label{tab:hyp_list}
\end{table}

==> phq9_table.tex <==
% latex table generated in R 4.3.2 by xtable 1.8-4 package
% Sun Feb 18 15:09:23 2024
\begin{table}[ht]
\centering
\begin{tabular}{llrrll}
  \hline
Exposure & Decision & p-value & Estimate & CI (marginal) & CI (corrected) \\ 
  \hline
any activity & Rejected & 0.00 & -0.78 & (-1.37, -0.18) & (-1.37, -0.18) \\ 
  any sports & Rejected & 0.00 & -1.16 & (-1.79, -0.51) & (-1.79, -0.51) \\ 
  no sports & Not Rejected & 0.61 & -0.17 & (-0.94, 0.58) & (-1.07, 0.72) \\ 
  any contact & Rejected & 0.00 & -1.38 & (-2.07, -0.72) & (-2.12, -0.67) \\ 
  no contact & Not Rejected & 0.03 & -1.06 & (-2.15, 0.04) & (-2.34, 0.24) \\ 
  any collision & Not Rejected & 0.01 & -1.12 & (-2.10, -0.14) & (-2.28, 0.04) \\ 
  no collision & Rejected & 0.00 & -1.25 & (-2.04, -0.45) & (-2.18, -0.31) \\ 
   \hline
\end{tabular}
\caption{Hypothesis testing for depression score} 
\label{tab:phq9}
\end{table}

